A method to estimate stellar ages from kinematical data

We present a method to build a probability density function (pdf) for the age of a star based on its peculiar velocities $U$, $V$ and $W$ and its orbital eccentricity. The sample used in this work comes from the Geneva-Copenhagen Survey (GCS) which contains both the spatial velocities, orbital eccentricities and isochronal ages for about $14\,000$ stars. Using the GCS stars, we fitted the parameters that describe the relations between the distributions of kinematical properties and age. This parametrization allows us to obtain an age probability from the kinematical data. From this age pdf, we estimate an individual average age for the star using the most likely age and the expected age. We have obtained the stellar age pdf for the age of $9\,102$ stars from the GCS and have shown that the distribution of individual ages derived from our method is in good agreement with the distribution of isochronal ages. We also observe a decline in the mean metallicity with our ages for stars younger than 7 Gyr, similar to the one observed for isochronal ages. This method can be useful for the estimation of rough stellar ages for those stars that fall in areas of the HR diagram where isochrones are tightly crowded. As an example of this method, we estimate the age of Trappist-1, which is a M8V star, obtaining the age of $t(UVW) = 12.50(+0.29-6.23)$ Gyr.

==> Source (2)/table.tex <==

\begin{table*}
	\scriptsize
	\centering
	\caption{Kinematical ages obtained through methods $UVW$ (1), $eVW$ (2) and $eUW$ (3) for the first 75 sample stars.}
	\label{tab:results50}
	\begin{tabular}{p{1cm}>{\raggedleft\arraybackslash}p{0.35cm}>{\raggedleft\arraybackslash}p{0.35cm}>{\raggedleft\arraybackslash}p{0.35cm}>{\raggedleft\arraybackslash}p{0.3cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}>{\raggedright\arraybackslash}p{0.22cm}}
\hline \\[-0.1cm]
Name & $U$ & $V$ & $W$ & $e$ & $t^{(1)}_{\mathrm{E}}$ & $t^{(1)}_{\mathrm{MP}}$ & $t^{(1)}_{2.5}$ & $t^{(1)}_{16}$ & $t^{(1)}_{50}$ & $t^{(1)}_{84}$ & $t^{(1)}_{97.5}$ & $t^{(2)}_{\mathrm{E}}$ & $t^{(2)}_{\mathrm{MP}}$ & $t^{(2)}_{2.5}$ & $t^{(2)}_{16}$ & $t^{(2)}_{50}$ & $t^{(2)}_{84}$ & $t^{(2)}_{97.5}$ & $t^{(3)}_{\mathrm{E}}$ & $t^{(3)}_{\mathrm{MP}}$ & $t^{(3)}_{2.5}$ & $t^{(3)}_{16}$ & $t^{(3)}_{50}$ & $t^{(3)}_{84}$ & $t^{(3)}_{97.5}$\\[+0.15cm]
\hline \\
HD 23        & 40 & -22 & -16 & 0.16 & 6.5 & 3.5 & 1.4 & 2.8 & 6.0 & 10.4 & 13.3 & 6.2 & 2.9 & 1.1 & 2.5 & 5.7 & 10.2 & 13.2 & 5.7 & 2.6 & 1.1 & 2.3 & 5.0 & 9.5 & 13.0\\
HD 105       & -10 & -21 & -1 & 0.06 & 3.1 & 0.3 & 0.1 & 0.4 & 1.8 & 6.4 & 11.9 & 3.5 & 0.6 & 0.3 & 0.7 & 2.3 & 6.9 & 12.0 & 3.4 & 0.6 & 0.2 & 0.6 & 2.2 & 6.7 & 12.0\\
HD 153       & -22 & -46 & 3.0 & 0.17 & 7.1 & 4.5 & 1.3 & 3.1 & 6.9 & 11.3 & 13.5 & 6.9 & 3.6 & 1.4 & 3 & 6.5 & 11.0 & 13.5 & 7.0 & 5.0 & 1.3 & 3.1 & 6.7 & 11.1 & 13.5\\
HD 156       & -9 & -1 & -15 & 0.02 & 3.3 & 0.5 & 0.2 & 0.6 & 2.1 & 6.4 & 11.7 & 3.0 & 0.6 & 0.3 & 0.7 & 1.9 & 5.7 & 11.1 & 3.1 & 0.6 & 0.3 & 0.6 & 1.9 & 5.9 & 11.3\\
HD 189       & 37 & -31 & -7 & 0.17 & 6.9 & 4.2 & 1.6 & 3.2 & 6.5 & 10.9 & 13.4 & 6.3 & 2.6 & 0.8 & 2.3 & 5.8 & 10.5 & 13.3 & 6.4 & 3.4 & 1.3 & 2.8 & 5.9 & 10.3 & 13.3\\
HD 200       & -4 & -50 & -23 & 0.18 & 8.1 & 7.6 & 2.2 & 4.3 & 8.1 & 11.9 & 13.6 & 7.9 & 7.5 & 2.1 & 4.2 & 7.9 & 11.8 & 13.6 & 7.8 & 6.6 & 2.1 & 4.1 & 7.7 & 11.7 & 13.6\\
HD 203       & -11 & -15 & -10 & 0.04 & 1.8 & 0.1 & 0.0 & 0.1 & 0.5 & 3.5 & 10.2 & 0.7 & 0.2 & 0.0 & 0.1 & 0.2 & 0.8 & 5.5 & 1.0 & 0.2 & 0.0 & 0.1 & 0.3 & 1.3 & 8.2\\
HD 268       & -28 & -50 & -18 & 0.19 & 7.7 & 6.6 & 1.6 & 3.7 & 7.6 & 11.7 & 13.6 & 7.4 & 5.4 & 1.7 & 3.6 & 7.3 & 11.5 & 13.6 & 7.5 & 5.3 & 1.6 & 3.6 & 7.4 & 11.5 & 13.6\\
HD 276       & -15 & -29 & -18 & 0.1 & 4.9 & 1.1 & 0.5 & 1.3 & 3.9 & 9.0 & 12.9 & 4.5 & 1.0 & 0.5 & 1.2 & 3.5 & 8.3 & 12.6 & 5.0 & 1.3 & 0.6 & 1.5 & 4.1 & 9.0 & 12.9\\
HD 285       & -50 & -10 & -15 & 0.12 & 5.2 & 1.9 & 0.8 & 1.8 & 4.4 & 9.1 & 12.9 & 5.1 & 1.6 & 0.7 & 1.7 & 4.2 & 8.9 & 12.8 & 5.0 & 1.7 & 0.8 & 1.7 & 4.1 & 8.6 & 12.7\\
HD 291       & 46 & -7 & -14 & 0.17 & 5.8 & 2.6 & 1.0 & 2.3 & 5.1 & 9.7 & 13.1 & 6.1 & 3.2 & 1.3 & 2.6 & 5.6 & 10.0 & 13.1 & 5.6 & 2.5 & 1.0 & 2.2 & 4.9 & 9.4 & 13.0\\
HD 307       & 12 & -59 & 0 & 0.23 & 9.0 & 10.4 & 3.0 & 5.4 & 9.1 & 12.4 & 13.7 & 8.4 & 9.3 & 2.4 & 4.7 & 8.6 & 12.1 & 13.7 & 8.8 & 9.2 & 2.9 & 5.3 & 8.9 & 12.3 & 13.7\\
HD 330       & -7 & -57 & -32 & 0.21 & 9.2 & 11.1 & 3.3 & 5.8 & 9.4 & 12.5 & 13.8 & 9.1 & 10.6 & 3.1 & 5.6 & 9.3 & 12.4 & 13.7 & 9.0 & 10.1 & 3.2 & 5.6 & 9.2 & 12.4 & 13.7\\
HD 334       & 5 & 5 & 30 & 0.07 & 7.6 & 6.0 & 2.4 & 4.2 & 7.3 & 11.1 & 13.4 & 7.7 & 6.2 & 2.6 & 4.4 & 7.4 & 11.1 & 13.4 & 7.8 & 6.7 & 2.5 & 4.4 & 7.6 & 11.3 & 13.5\\
HD 373       & -25 & -18 & 5 & 0.07 & 4.2 & 0.8 & 0.4 & 1.0 & 3.1 & 8.0 & 12.5 & 4.3 & 0.9 & 0.5 & 1.1 & 3.3 & 7.9 & 12.4 & 4.5 & 0.9 & 0.5 & 1.3 & 3.6 & 8.3 & 12.6\\
HD 392       & -26 & -9 & -1 & 0.05 & 3.3 & 0.5 & 0.2 & 0.6 & 2.1 & 6.5 & 11.8 & 3.3 & 0.6 & 0.3 & 0.6 & 2.1 & 6.5 & 11.8 & 3.1 & 0.6 & 0.3 & 0.7 & 2.0 & 5.9 & 11.4\\
HD 427       & -11 & 3 & 19 & 0.04 & 6.3 & 3.6 & 1.5 & 2.9 & 5.7 & 9.9 & 13.1 & 5.9 & 3.3 & 1.4 & 2.7 & 5.3 & 9.4 & 12.9 & 6.4 & 3.7 & 1.5 & 2.9 & 5.9 & 10.2 & 13.2\\
HD 439       & -44 & -57 & -7 & 0.23 & 8.4 & 9.9 & 2.1 & 4.5 & 8.5 & 12.2 & 13.7 & 8.4 & 9.4 & 2.3 & 4.7 & 8.5 & 12.1 & 13.7 & 8.1 & 8.0 & 1.9 & 4.3 & 8.2 & 12.0 & 13.7\\
HD 447       & -12 & 11 & -1 & 0.06 & 4.5 & 1.5 & 0.6 & 1.4 & 3.6 & 7.9 & 12.3 & 4.4 & 1.4 & 0.6 & 1.4 & 3.5 & 7.7 & 12.1 & 3.4 & 0.6 & 0.2 & 0.6 & 2.1 & 6.7 & 11.9\\
HD 457       & -31 & -17 & 14 & 0.07 & 5.9 & 2.6 & 1.1 & 2.3 & 5.2 & 9.8 & 13.1 & 5.8 & 2.6 & 1.1 & 2.3 & 5.2 & 9.7 & 13.0 & 5.5 & 2.5 & 1.1 & 2.2 & 4.8 & 9.2 & 12.9\\
HD 466       & -21 & -18 & 13 & 0.06 & 5.6 & 2.1 & 0.9 & 2.0 & 4.8 & 9.5 & 13 & 5.1 & 1.9 & 0.9 & 1.8 & 4.3 & 8.9 & 12.8 & 5.7 & 2.4 & 1.0 & 2.2 & 5.0 & 9.5 & 13.0\\
HD 547       & -22 & -63 & -12 & 0.24 & 9.0 & 11.2 & 2.8 & 5.4 & 9.2 & 12.4 & 13.8 & 8.8 & 10.1 & 2.7 & 5.2 & 9.0 & 12.3 & 13.7 & 8.8 & 9.6 & 2.7 & 5.2 & 9.0 & 12.4 & 13.7\\
HD 564       & 27 & 4 & -4 & 0.11 & 4.1 & 0.8 & 0.3 & 1.0 & 3.0 & 7.6 & 12.2 & 4.4 & 0.8 & 0.5 & 1.3 & 3.6 & 8.0 & 12.3 & 3.8 & 0.8 & 0.4 & 0.9 & 2.7 & 7.1 & 12.1\\
HD 578       & 26 & -3 & 18 & 0.11 & 6.5 & 3.8 & 1.5 & 3.0 & 6.0 & 10.3 & 13.2 & 6.7 & 4.2 & 1.7 & 3.2 & 6.3 & 10.4 & 13.2 & 6.3 & 3.6 & 1.5 & 2.9 & 5.8 & 10.0 & 13.2\\
HD 604       & -18 & -38 & -15 & 0.13 & 5.9 & 1.8 & 0.7 & 1.9 & 5.2 & 10.1 & 13.2 & 6.0 & 2.0 & 0.9 & 2.2 & 5.4 & 10.2 & 13.3 & 5.5 & 1.7 & 0.7 & 1.8 & 4.8 & 9.7 & 13.1\\
HD 610       & 1 & -11 & -6 & 0.04 & 1.8 & 0.1 & 0.0 & 0.1 & 0.6 & 3.7 & 10.2 & 1.0 & 0.2 & 0.0 & 0.1 & 0.3 & 1.3 & 7.6 & 0.9 & 0.2 & 0.0 & 0.1 & 0.3 & 1.3 & 6.8\\
HD 615       & 34 & -5 & -8 & 0.13 & 4.6 & 1.3 & 0.5 & 1.3 & 3.6 & 8.3 & 12.6 & 5.0 & 1.7 & 0.6 & 1.6 & 4.1 & 8.7 & 12.7 & 4.4 & 1.2 & 0.5 & 1.3 & 3.4 & 7.9 & 12.4\\
HD 631       & -14 & 11 & -30 & 0.07 & 6.2 & 3.6 & 1.5 & 2.8 & 5.6 & 9.8 & 13.0 & 5.7 & 3.2 & 1.3 & 2.6 & 5.1 & 9.1 & 12.7 & 6.1 & 3.2 & 1.3 & 2.6 & 5.6 & 10.0 & 13.2\\
HD 633       & -1 & 13 & -12 & 0.08 & 4.4 & 1.3 & 0.5 & 1.3 & 3.4 & 7.8 & 12.2 & 4.1 & 1.3 & 0.6 & 1.3 & 3.2 & 7.1 & 11.7 & 3.9 & 0.7 & 0.4 & 0.9 & 2.8 & 7.6 & 12.3\\
HD 700       & 3 & 11 & 5 & 0.08 & 4.8 & 1.6 & 0.7 & 1.6 & 3.9 & 8.3 & 12.5 & 4.8 & 2.0 & 0.8 & 1.8 & 4.0 & 8.1 & 12.3 & 4.8 & 1.4 & 0.6 & 1.5 & 3.9 & 8.7 & 12.7\\
HD 732       & -26 & -14 & -2 & 0.06 & 2.9 & 0.3 & 0.1 & 0.4 & 1.6 & 5.9 & 11.6 & 3.2 & 0.6 & 0.2 & 0.6 & 2.0 & 6.5 & 11.8 & 3.2 & 0.6 & 0.2 & 0.7 & 2.1 & 6.3 & 11.6\\
HD 804       & -33 & -63 & 20 & 0.24 & 9.7 & 13.0 & 3.8 & 6.5 & 10.0 & 12.8 & 13.8 & 9.5 & 12.5 & 3.7 & 6.3 & 9.9 & 12.7 & 13.8 & 9.5 & 12.4 & 3.6 & 6.3 & 9.8 & 12.7 & 13.8\\
HD 852       & -29 & -17 & -6 & 0.07 & 2.6 & 0.1 & 0.0 & 0.2 & 1.2 & 5.5 & 11.5 & 2.4 & 0.2 & 0.1 & 0.2 & 1.1 & 5.2 & 11.2 & 3.0 & 0.2 & 0.1 & 0.4 & 1.8 & 5.9 & 11.4\\
HD 900       & -8 & -3 & -19 & 0.01 & 3.9 & 0.8 & 0.4 & 0.9 & 2.7 & 7.2 & 12.1 & 3.5 & 0.7 & 0.4 & 0.8 & 2.4 & 6.5 & 11.6 & 3.3 & 0.7 & 0.4 & 0.8 & 2.2 & 6.2 & 11.5\\
HD 903       & -22 & -9 & 7 & 0.04 & 4.4 & 1.2 & 0.5 & 1.2 & 3.4 & 8.0 & 12.5 & 4.4 & 1.1 & 0.5 & 1.3 & 3.5 & 8.0 & 12.4 & 4.1 & 1.2 & 0.5 & 1.2 & 3.1 & 7.4 & 12.1\\
HD 912       & -38 & -10 & -1 & 0.08 & 4.2 & 0.9 & 0.4 & 1.0 & 3.1 & 7.8 & 12.4 & 3.9 & 0.7 & 0.4 & 0.9 & 2.8 & 7.4 & 12.2 & 4.1 & 1.0 & 0.5 & 1.1 & 3.1 & 7.5 & 12.2\\
HD 949       & -32 & -12 & 4 & 0.07 & 4.3 & 1.0 & 0.4 & 1.1 & 3.3 & 8.0 & 12.5 & 4.3 & 0.9 & 0.5 & 1.1 & 3.3 & 8.1 & 12.5 & 4.1 & 1.1 & 0.5 & 1.2 & 3.1 & 7.5 & 12.2\\
HD 975       & -4 & 3 & 1 & 0.04 & 3.6 & 0.7 & 0.3 & 0.8 & 2.5 & 6.8 & 11.9 & 3.4 & 0.7 & 0.4 & 0.9 & 2.4 & 6.3 & 11.3 & 3.4 & 0.6 & 0.3 & 0.7 & 2.2 & 6.5 & 11.8\\
HD 984       & -13 & -24 & -6 & 0.08 & 2.9 & 0.2 & 0.1 & 0.3 & 1.5 & 6.1 & 11.8 & 2.4 & 0.2 & 0.1 & 0.3 & 1.2 & 5.0 & 11.1 & 3.3 & 0.3 & 0.1 & 0.4 & 2.0 & 6.7 & 12.0\\
HD 1000      & 46 & -46 & 10 & 0.23 & 9.0 & 9.6 & 3.3 & 5.6 & 9.0 & 12.3 & 13.7 & 8.7 & 10.4 & 2.5 & 5.1 & 8.9 & 12.3 & 13.7 & 8.6 & 8.2 & 3.0 & 5.2 & 8.7 & 12.1 & 13.7\\
HD 1004      & 9 & -11 & -12 & 0.06 & 3.0 & 0.3 & 0.1 & 0.4 & 1.7 & 5.9 & 11.6 & 3.3 & 0.6 & 0.3 & 0.6 & 2.0 & 6.6 & 11.9 & 2.6 & 0.6 & 0.2 & 0.5 & 1.4 & 5.0 & 10.8\\
HD 1015      & 46 & -24 & -8 & 0.18 & 6.8 & 4.0 & 1.6 & 3.1 & 6.4 & 10.7 & 13.4 & 6.4 & 3.5 & 1.2 & 2.7 & 6.0 & 10.5 & 13.3 & 6.0 & 3.0 & 1.2 & 2.5 & 5.4 & 9.9 & 13.1\\
HD 1047      & 0 & 11 & 0 & 0.07 & 4.3 & 1.2 & 0.5 & 1.2 & 3.3 & 7.7 & 12.2 & 4.0 & 1.2 & 0.5 & 1.3 & 3.1 & 7.0 & 11.7 & 3.9 & 0.7 & 0.4 & 0.9 & 2.8 & 7.5 & 12.3\\
HD 1094      & -13 & -15 & -44 & 0.03 & 7.7 & 6.1 & 2.3 & 4.2 & 7.5 & 11.3 & 13.5 & 8.0 & 7.3 & 2.7 & 4.7 & 7.9 & 11.5 & 13.5 & 7.5 & 5.7 & 2.4 & 4.2 & 7.3 & 11.1 & 13.4\\
HD 1101      & -12 & -23 & -6 & 0.07 & 2.7 & 0.2 & 0.0 & 0.2 & 1.3 & 5.7 & 11.7 & 2.7 & 0.2 & 0.1 & 0.3 & 1.4 & 5.7 & 11.5 & 2.5 & 0.2 & 0.1 & 0.2 & 1.1 & 5.4 & 11.3\\
HD 1184      & 42 & -17 & -41 & 0.16 & 8.3 & 7.3 & 2.8 & 4.8 & 8.1 & 11.7 & 13.6 & 8.2 & 7.5 & 2.8 & 4.8 & 8.2 & 11.7 & 13.6 & 7.8 & 6.8 & 2.6 & 4.4 & 7.6 & 11.4 & 13.5\\
HD 1204      & 35 & -42 & -23 & 0.2 & 8.3 & 7.6 & 2.6 & 4.7 & 8.2 & 11.9 & 13.6 & 8.0 & 8.0 & 2.0 & 4.2 & 8.1 & 11.9 & 13.6 & 8.0 & 6.9 & 2.4 & 4.5 & 7.9 & 11.7 & 13.6\\
HD 1213      & -24 & -12 & 3 & 0.05 & 3.7 & 0.6 & 0.3 & 0.8 & 2.6 & 7.2 & 12.2 & 3.8 & 0.7 & 0.4 & 0.8 & 2.7 & 7.2 & 12.1 & 3.6 & 0.7 & 0.4 & 0.9 & 2.6 & 6.8 & 11.8\\
HD 1271      & -45 & -53 & 38 & 0.21 & 10.2 & 13.4 & 4.6 & 7.3 & 10.5 & 12.9 & 13.8 & 10.0 & 12.5 & 4.5 & 7.1 & 10.3 & 12.8 & 13.8 & 9.9 & 11.6 & 4.4 & 7.0 & 10.2 & 12.8 & 13.8\\
HD 1343      & -4 & -3 & 3 & 0.02 & 3.5 & 0.6 & 0.3 & 0.7 & 2.4 & 6.7 & 11.9 & 3.4 & 0.7 & 0.4 & 0.8 & 2.4 & 6.4 & 11.5 & 3.1 & 0.6 & 0.3 & 0.7 & 1.9 & 5.9 & 11.3\\
HD 1352      & -40 & -21 & -16 & 0.11 & 4.6 & 0.9 & 0.4 & 1.1 & 3.5 & 8.5 & 12.7 & 4.9 & 1.2 & 0.5 & 1.4 & 4.0 & 9.0 & 12.9 & 4.8 & 1.5 & 0.5 & 1.4 & 4.0 & 8.7 & 12.7\\
HD 1391      & 12 & 1 & -8 & 0.07 & 2.8 & 0.3 & 0.1 & 0.4 & 1.6 & 5.7 & 11.3 & 3.5 & 0.6 & 0.2 & 0.7 & 2.4 & 6.7 & 11.8 & 2.4 & 0.3 & 0.1 & 0.4 & 1.3 & 4.8 & 10.7\\
HD 1418      & 13 & -35 & -42 & 0.13 & 8.6 & 8.3 & 2.9 & 5.1 & 8.5 & 12.0 & 13.7 & 8.1 & 7.0 & 2.6 & 4.6 & 8.0 & 11.7 & 13.6 & 8.2 & 6.9 & 2.8 & 4.8 & 8.2 & 11.8 & 13.6\\
HD 1455      & 19 & -15 & 3 & 0.09 & 4.7 & 1.3 & 0.6 & 1.4 & 3.7 & 8.5 & 12.7 & 4.6 & 1.1 & 0.5 & 1.3 & 3.6 & 8.5 & 12.7 & 3.9 & 0.9 & 0.4 & 1.0 & 2.9 & 7.2 & 12.1\\
HD 1497      & 14 & -27 & -17 & 0.11 & 5.6 & 2.0 & 0.8 & 1.9 & 4.8 & 9.6 & 13.1 & 5.0 & 1.3 & 0.6 & 1.5 & 4.2 & 9.1 & 12.9 & 5.3 & 1.9 & 0.8 & 1.8 & 4.5 & 9.2 & 12.9\\
HD 1513      & 3 & -2 & -2 & 0.04 & 2.7 & 0.3 & 0.1 & 0.3 & 1.4 & 5.4 & 11.2 & 3.2 & 0.6 & 0.2 & 0.6 & 2.1 & 6.3 & 11.6 & 2.2 & 0.3 & 0.1 & 0.3 & 1.1 & 4.4 & 10.4\\
HD 1557      & -47 & 6 & -32 & 0.12 & 7.1 & 5.0 & 2.0 & 3.7 & 6.7 & 10.6 & 13.3 & 6.7 & 4.4 & 1.8 & 3.3 & 6.3 & 10.3 & 13.2 & 6.7 & 4.1 & 1.7 & 3.2 & 6.2 & 10.4 & 13.2\\
HD 1591      & -36 & -21 & -9 & 0.1 & 3.5 & 0.3 & 0.1 & 0.5 & 2.1 & 7.0 & 12.2 & 4.1 & 0.6 & 0.3 & 0.8 & 2.9 & 8.0 & 12.5 & 4.0 & 0.6 & 0.3 & 0.8 & 2.9 & 7.7 & 12.4\\
HD 1603      & 24 & -7 & -2 & 0.1 & 4.0 & 0.8 & 0.3 & 1.0 & 2.9 & 7.6 & 12.3 & 4.3 & 0.9 & 0.5 & 1.2 & 3.4 & 8.0 & 12.4 & 3.7 & 0.7 & 0.4 & 0.9 & 2.6 & 7.0 & 12.0\\
HD 1674      & 54 & -7 & 12 & 0.19 & 7.1 & 4.9 & 1.9 & 3.6 & 6.8 & 10.9 & 13.4 & 7.3 & 5.5 & 2.0 & 3.8 & 7.0 & 10.9 & 13.4 & 7.0 & 4.2 & 1.8 & 3.5 & 6.6 & 10.8 & 13.4\\
HD 1683      & 29 & -5 & -2 & 0.12 & 4.4 & 1.1 & 0.4 & 1.2 & 3.3 & 8.0 & 12.5 & 4.8 & 1.4 & 0.6 & 1.5 & 4.0 & 8.6 & 12.6 & 4.1 & 1.1 & 0.5 & 1.2 & 3.1 & 7.6 & 12.3\\
HD 1686      & 11 & 4 & -6 & 0.07 & 3.1 & 0.4 & 0.1 & 0.5 & 1.9 & 6.1 & 11.5 & 3.7 & 0.6 & 0.3 & 0.8 & 2.7 & 7.0 & 11.9 & 2.6 & 0.5 & 0.1 & 0.5 & 1.5 & 5.1 & 10.9\\
HD 1689      & -22 & 16 & 3 & 0.09 & 5.6 & 2.8 & 1.1 & 2.3 & 4.9 & 9.1 & 12.8 & 4.7 & 2.0 & 0.9 & 1.8 & 3.9 & 7.9 & 12.1 & 4.5 & 0.7 & 0.4 & 1.1 & 3.5 & 8.4 & 12.7\\
HD 1764      & -1 & -41 & 8 & 0.15 & 7.1 & 4.5 & 1.5 & 3.3 & 6.8 & 11.2 & 13.5 & 6.6 & 3.4 & 1.3 & 2.8 & 6.2 & 10.7 & 13.4 & 7.0 & 4.5 & 1.6 & 3.3 & 6.7 & 11.0 & 13.4\\
HD 1778      & 50 & -16 & -23 & 0.18 & 7.1 & 4.6 & 1.8 & 3.4 & 6.7 & 10.9 & 13.4 & 7.0 & 4.2 & 1.7 & 3.4 & 6.7 & 10.8 & 13.4 & 6.5 & 3.9 & 1.5 & 3.0 & 6.0 & 10.3 & 13.2\\
HD 1828      & -10 & -4 & -24 & 0.01 & 4.7 & 1.5 & 0.7 & 1.5 & 3.8 & 8.3 & 12.6 & 4.2 & 1.2 & 0.6 & 1.3 & 3.3 & 7.5 & 12.1 & 4.1 & 1.2 & 0.6 & 1.3 & 3.2 & 7.4 & 12.1\\
HD 1856      & -25 & -28 & -15 & 0.1 & 4.3 & 0.6 & 0.3 & 0.9 & 3.1 & 8.3 & 12.7 & 4.0 & 0.7 & 0.4 & 0.9 & 2.9 & 7.7 & 12.4 & 4.4 & 0.7 & 0.4 & 1.0 & 3.4 & 8.4 & 12.7\\
HD 1898      & 33 & 6 & -8 & 0.14 & 4.5 & 1.2 & 0.5 & 1.2 & 3.5 & 8.1 & 12.5 & 5.1 & 1.6 & 0.7 & 1.7 & 4.4 & 8.8 & 12.6 & 4.9 & 1.8 & 0.7 & 1.6 & 4.0 & 8.6 & 12.7\\
HD 1952      & 14 & -8 & 2 & 0.07 & 3.8 & 0.7 & 0.3 & 0.9 & 2.7 & 7.3 & 12.2 & 4.0 & 0.8 & 0.4 & 1.0 & 3.0 & 7.6 & 12.3 & 3.5 & 0.7 & 0.4 & 0.8 & 2.4 & 6.6 & 11.8\\
HD 1980      & -34 & -7 & 6 & 0.07 & 4.9 & 1.6 & 0.7 & 1.6 & 3.9 & 8.6 & 12.7 & 4.6 & 1.3 & 0.6 & 1.4 & 3.7 & 8.3 & 12.6 & 4.5 & 1.4 & 0.6 & 1.5 & 3.6 & 8.1 & 12.4\\
HD 2021      & -15 & -4 & -12 & 0.02 & 2.8 & 0.3 & 0.1 & 0.4 & 1.6 & 5.6 & 11.3 & 2.7 & 0.4 & 0.1 & 0.5 & 1.6 & 5.3 & 10.9 & 2.3 & 0.3 & 0.1 & 0.4 & 1.2 & 4.5 & 10.4\\
HD 2121      & -53 & -30 & 9 & 0.16 & 6.6 & 3.3 & 1.2 & 2.7 & 6.2 & 10.8 & 13.4 & 6.9 & 4.1 & 1.4 & 3.1 & 6.6 & 11 & 13.4 & 6.7 & 4.1 & 1.3 & 3.0 & 6.4 & 10.7 & 13.4\\
HD 2302      & -29 & -23 & -8 & 0.09 & 2.9 & 0.2 & 0.0 & 0.3 & 1.5 & 6.2 & 11.9 & 3.1 & 0.2 & 0.1 & 0.3 & 1.8 & 6.5 & 11.9 & 3.1 & 0.2 & 0.1 & 0.3 & 1.8 & 6.6 & 12.0\\
HD 2305      & -3 & -16 & -10 & 0.05 & 2.2 & 0.1 & 0.0 & 0.1 & 0.9 & 4.5 & 10.9 & 0.8 & 0.2 & 0.0 & 0.1 & 0.3 & 1.1 & 6.6 & 2.1 & 0.2 & 0.1 & 0.2 & 0.9 & 4.6 & 10.8\\
HD 2330      & -6 & -25 & -12 & 0.08 & 3.7 & 0.5 & 0.2 & 0.7 & 2.5 & 7.4 & 12.4 & 3.3 & 0.6 & 0.3 & 0.7 & 2.1 & 6.7 & 12.0 & 3.9 & 0.6 & 0.4 & 0.8 & 2.7 & 7.5 & 12.3\\[+0.10cm]
		\hline
	\end{tabular}
\end{table*}
